Towards a Hands-Free Query Optimizer through Deep Learning

Query optimization remains one of the most important and well-studied problems in database systems. However, traditional query optimizers are complex heuristically-driven systems, requiring large amounts of time to tune for a particular database and requiring even more time to develop and maintain in the first place. In this vision paper, we argue that a new type of query optimizer, based on deep reinforcement learning, can drastically improve on the state-of-the-art. We identify potential complications for future research that integrates deep learning with query optimization, and we describe three novel deep learning based approaches that can lead the way to end-to-end learning-based query optimizers.

==> searchspace.tex <==
\section{Challenge 1: End-to-End Learning} \label{sec:searchspace}

While ReJOIN demonstrates that ability for \DRL algorithms to find good policies in extremely large search spaces (e.g., there are over 500 billion possible join orderings for a query with 10 relations), the entire search space for execution plans is still significantly larger. Accounting for operator selection, access path selection, potential concurrency, locking strategies, etc. create such a large search space that the ReJOIN approach cannot be easily scaled up. Theoretical results~\cite{near_opt_rl} suggest that adding additional non-trivial dimensions to the problem -- such as operator selection -- increases convergence time drastically. %If query latency were used as a reward signal for a fully end-to-end \DRL-driven query optimizer in the style of ReJOIN, convergence time would undoubtedly be prohibitive.

